Ain't Misbehavin' -- Using LLMs to Generate Expressive Robot Behavior in Conversations with the Tabletop Robot Haru

Social robots aim to establish long-term bonds with humans through engaging conversation. However, traditional conversational approaches, reliant on scripted interactions, often fall short in maintaining engaging conversations. This paper addresses this limitation by integrating large language models (LLMs) into social robots to achieve more dynamic and expressive conversations. We introduce a fully-automated conversation system that leverages LLMs to generate robot responses with expressive behaviors, congruent with the robot's personality. We incorporate robot behavior with two modalities: 1) a text-to-speech (TTS) engine capable of various delivery styles, and 2) a library of physical actions for the robot. We develop a custom, state-of-the-art emotion recognition model to dynamically select the robot's tone of voice and utilize emojis from LLM output as cues for generating robot actions. A demo of our system is available here. To illuminate design and implementation issues, we conduct a pilot study where volunteers chat with a social robot using our proposed system, and we analyze their feedback, conducting a rigorous error analysis of chat transcripts. Feedback was overwhelmingly positive, with participants commenting on the robot's empathy, helpfulness, naturalness, and entertainment. Most negative feedback was due to automatic speech recognition (ASR) errors which had limited impact on conversations. However, we observed a small class of errors, such as the LLM repeating itself or hallucinating fictitious information and human responses, that have the potential to derail conversations, raising important issues for LLM application.

==> section/1_introduction.tex <==
%\vspace*{-2mm}
\section{Introduction}
\label{sec:intro}
 
%  Common approaches, primarily based on predefined scripts and topics, often lead to monotonous, repetitive human-robot dialogues over time. This paper addresses this limitation by integrating conversation-oriented LLMs into social robots, aiming to enrich user experience through more fluid and responsive interactions.

% The recent advancements in the capabilities and accessibility of LLMs offer great possibilities for social robotics. These models excel in processing open-ended instructions and maintaining conversational context, making them ideal for dialogues, as evident in applications like chatbots and virtual agents. However, the integration of LLMs in social robots presents unique challenges. Unlike virtual agents, social robots possess physical embodiment and distinct personalities. Their effectiveness and likability hinge not only on conveying comprehension through words but also on exhibiting appropriate expressive robot behavior, such as body language and tone of voice. The expressivity of social robots is key to conveying believable emotions, and it is challenging to generate appropriate emotive behavior on the fly when working with conversational content generated by an LLM.

% This research aims to determine how to automatically generate expressive robot behaviors in conversations where the robot's utterances are generated by an LLM.  To tackle the research question, we developed an LLM-driven conversation system with a robot behavior generation module for our social robot, Haru. The system incorporates two methods for rendering robot behavior: 1) An adaptive text-to-speech engine capable of various delivery styles, and 2) Physical actions executed by the robot. This innovative system dynamically generates responses in alignment with Haru's personality and employs an advanced textual emotion recognition model to pick the robot's tone of voice. Furthermore, we utilized emojis from LLM outputs as cues for the robot's physical actions. We conducted experiments with a real robot and human conversants, to evaluate the effectiveness of our approach. Since the LLM by nature is still inconsistent, We performed error-analysis from the experiential logs and participants feedback. Small errors in LLM or the input, caused detrimental effects on how user perceives the robot. We explored new challenges to integrate LLM in social robots. This will be integral factors to be considered in order to develop a successful application using LLM in social robots. 

% in terms of expressivity characteristics, robot personality traits measured by RoSAS (Robot Social Attributes Scale), and rapport expectation via RERS (Rapport Expectation Rating Scale). 

%Text-based collaborative storytelling games have been tested. In particular, \cite{nichols2020mig} formulated a text-based version of an \cst~game and \cite{nichols2021iros} evaluated it, conducting an elicitation study for a hypothetical social robot version the game. But evaluation of text-based interfaces, however thorough, offers a limited view of the challenges that will arise when the game is played with a social robot in real-world scenarios.


==> tbl/error_analysis.tex <==
\begin{tabular}{lc}
\textbf{Category} & \textbf{Count} \\
\hline
LLM problems & 10 \\
ASR problems & 4 \\
Short interaction & 4 \\
Boring conversation topic & 4 \\
Excessive actions & 4 \\
Robot lack of guidance and self-disclosure & 3 \\
\hline
\end{tabular}

